Enhancing Travel Decision-Making: A Contrastive Learning Approach for Personalized Review Rankings in Accommodations

User-generated reviews significantly influence consumer decisions, particularly in the travel domain when selecting accommodations. This paper contribution comprising two main elements. Firstly, we present a novel dataset of authentic guest reviews sourced from a prominent online travel platform, totaling over two million reviews from 50,000 distinct accommodations. Secondly, we propose an innovative approach for personalized review ranking. Our method employs contrastive learning to intricately capture the relationship between a review and the contextual information of its respective reviewer. Through a comprehensive experimental study, we demonstrate that our approach surpasses several baselines across all reported metrics. Augmented by a comparative analysis, we showcase the efficacy of our method in elevating personalized review ranking. The implications of our research extend beyond the travel domain, with potential applications in other sectors where personalized review ranking is paramount, such as online e-commerce platforms.

==> drafts/abstracts.tex <==
% \eran{original abstract:
% Online reviews play a crucial role in consumer decision-making, but traditional review ranking models often fall short in providing personalized recommendations. This paper addresses the limitations of existing approaches by introducing a novel personalized reviews ranking model. Our methodology leverages contrastive learning to capture the intricate relationship between users and reviews, acknowledging diverse user perspectives. We present experimental results demonstrating the efficacy of our approach in enhancing the accuracy of personalized review rankings, mitigating biases, and providing a nuanced understanding of user preferences. Our contributions include a novel contrastive learning framework and insights into the challenges of personalized reviews ranking. This work has significant implications for improving user satisfaction and decision-making in online review platforms.}

% \moran{new suggested abstract:
% Users' reviews significantly influence consumer decisions, particularly in the travel domain when selecting accommodations. However, traditional review ranking models often lack in delivering personalized recommendations. This paper presents a new reviews dataset from Booking.com. tackles the limitations of existing approaches by introducing a pioneering personalized reviews ranking approach. Our methodology employs contrastive learning to comprehend the intricate dynamics between users and reviews, accommodating diverse user perspectives. Through experiments, we showcase how our approach effectively improves the accuracy of personalized review rankings, reduces biases, and fosters a nuanced understanding of user preferences. Our contributions encompass a unique contrastive learning framework and valuable insights into the challenges associated with personalized review ranking. This research bears significant implications for enhancing user satisfaction and decision-making within online e-commerce platforms.}

